Toward Parametric Timed Interfaces for Real-Time Components

We propose here a framework to model real-time components consisting of concurrent real-time tasks running on a single processor, using parametric timed automata. Our framework is generic and modular, so as to be easily adapted to different schedulers and more complex task models. We first perform a parametric schedulability analysis of the components using the inverse method. We show that the method unfortunately does not provide satisfactory results when the task periods are consid- ered as parameters. After identifying and explaining the problem, we present a solution adapting the model by making use of the worst-case scenario in schedulability analysis. We show that the analysis with the inverse method always converges on the modified model when the system load is strictly less than 100%. Finally, we show how to use our parametric analysis for the generation of timed interfaces in compositional system design.

==> eptcsdata.tex <==
\providecommand{\firstpage}{49}
\providecommand{\publicationstatus}{\'E. Andr\'e and G. Frehse (Eds.): 1st International Workshop\\ on Synthesis of Continuous Parameters (SynCoP'14).\\
EPTCS 145, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.145.6}{10.4204/EPTCS.145.6}}
\pdfoutput=1

